CHAMELEON: OutSystems Live Bidirectional Transformations

In model-driven engineering, the bidirectional transformation of models plays a crucial role in facilitating the use of editors that operate at different levels of abstraction. This is particularly important in the context of industrial-grade low-code platforms like OutSystems, which feature a comprehensive ecosystem of tools that complement the standard integrated development environment with domain-specific builders and abstract model viewers. We introduce CHAMELEON, a tool that enables the dynamic definition of a live bidirectional model transformation in a declarative manner by leveraging simple and intuitive component patterns. Through this approach, we can gradually define the view and synthesis paths to an abstract model built on top of a low-code metamodel. We devise a standard parser-generating technique for tree-like models that builds upon extended grammar definitions with constraints and name binders. We allow for a greater overlap of model patterns that can still be disambiguated for a clear lens-like behaviour of the transformation. CHAMELEON is evaluated in the fragment of the OutSystems language targeting the definition of user interfaces. To assess performance we used a large set of real OutSystems applications, with approximately 200K UI widgets, and a database of curated widget patterns. We found a worst-case processing time of 92ms for complete models in our benchmark, which is still suitable for the operation of an interactive model editor.

==> example/output/EnumInput.tex <==
%!TEX root = ../../main-ieee.tex
\begin{tabular}{l}
\hline
\multicolumn{1}{c}{EnumInput(Expression \kw{Variable}, string \kw{Label} = \kw{GetLabelFor(Value)})}\\
\hline
    \textbf{Pattern\#1}\\
    \kw{Variable} = \kw{i.Variable}\\
    \kw{Label} = \kw{t.Value}\\
  \hline
    \begin{lstlisting}[basicstyle=\footnotesize\ttfamily,language=XML,numbers=none,frame=none,gobble=6,boxpos=t]
      <Label>
        <Text Id="t"/>
      </Label>
      <ButtonGroup Id="i">
        <ButtonGroupItem>
          <Text/>
        </ButtonGroupItem>
      </ButtonGroup>
    \end{lstlisting}
  \\ \hline
    \includegraphics[width=.15 \linewidth]{figures/EnumInput.1.png}
  \\ \hline
\end{tabular}

